RoboUniverse-10K: Toward the Scaling Era of Agentic Robotics via Real-to-Sim Environments

Agentic Robotics, in which foundation models act as coding agents to control robots through executable programs, has emerged as a compelling paradigm for embodied intelligence. Yet unlike software engineering, where massive executable environments power post-training, robotics remains constrained by small, manual benchmarks and in-distribution evaluation. To bridge this gap, we introduce RoboUniverse-10K, 10,807 interactive, resettable, and verifiable physics environments built from real-world videos via an automated Real2Sim and quality assurance pipeline. Each runs in an isolated, Harbor-compatible harness that hides privileged states and grading logic to mirror real-world sensing. From the same pipeline, we hold out 500 unseen tasks to establish RoboUniverse-Verified, an expert-verified zero-shot benchmark. Evaluating 11 closed- and open-source models reveals a huge gap: frontier models reach 85.8\% success, while open-source baselines lag at 2.6\% to 10.0\%, bottlenecked by low-level grasping, deformable-object manipulation, and post-contact physical control. Finally, we collect about 17K multi-turn trajectories totaling 0.79B tokens with GPT-6 Astra and perform full-parameter supervised fine-tuning on Qwen3.6-35B-A3B, yielding RoboUniverse-35B-A3B. Our model achieves substantial zero-shot gains on RoboUniverse-Verified, lifting the success rate from 0.8\% to 21.2\%, while achieving zero-shot task completions across LIBERO-MAX, RoboCasa, RoboTwin 2.0, and a real Franka arm. We open-source the RL-ready environments and model to lay the foundation for large-scale reinforcement learning in Agentic Robotics.

==> style/questionbox.tex <==
% Question callout matching the Chinese manuscript.
\definecolor{questionframe}{HTML}{4C42F5}
\definecolor{questionbackground}{HTML}{F3F2FF}
\newtcolorbox{questionbox}{colback=questionbackground,colframe=questionframe,
  coltext=black,boxrule=0.8pt,arc=3pt,left=9pt,right=9pt,top=5pt,bottom=5pt,
  before skip=7pt,after skip=8pt}

